On Rollouts in Model-Based Reinforcement Learning

Model-based reinforcement learning (MBRL) seeks to enhance data efficiency by learning a model of the environment and generating synthetic rollouts from it. However, accumulated model errors during these rollouts can distort the data distribution, negatively impacting policy learning and hindering long-term planning. Thus, the accumulation of model errors is a key bottleneck in current MBRL methods. We propose Infoprop, a model-based rollout mechanism that separates aleatoric from epistemic model uncertainty and reduces the influence of the latter on the data distribution. Further, Infoprop keeps track of accumulated model errors along a model rollout and provides termination criteria to limit data corruption. We demonstrate the capabilities of Infoprop in the Infoprop-Dyna algorithm, reporting state-of-the-art performance in Dyna-style MBRL on common MuJoCo benchmark tasks while substantially increasing rollout length and data quality.

==> sections/99_backup.tex <==


%\begin{comment}
\subsection{Information-Theoretic Relation between Environment and Model}
\label{sec_ip_theory}

To introduce an interdependence between $\rvenvnextstate$ in \eqref{eq:env_prediction} and $\rvmodnextstate$ in \eqref{eq:TS_prediction} we define an error process $\rvmoderror$.

\begin{definition}
    \label{def:error_process}
    We introduce a model error $\rvmoderror \sim \moderrordist$, such that $\rvmodnextstate = \rvenvnextstate + \Delta_t$. Thus, $\rvmoderror$ maps the uncertainty in the parameter space $\distparams$ to the output space of the model. In the following, we are solely concerned with the first two moments of $\moderrordist$, such that
    \begin{equation}
        \rvmodnextstate = \rvenvnextstate + \modbias(\rvgenstate, \rvgenact) + \epichol(\rvgenstate, \rvgenact) \rvmodepi
        \label{eq:error_proc}
    \end{equation}
    with $\epichol(\rvgenstate, \rvgenact)\epichol(\rvgenstate, \rvgenact)^\top = \epivar(\rvgenstate, \rvgenact)$ and $\rvmodepi \sim \gauss (0, I)$. We refer to $\modbias(\rvgenstate, \rvgenact)$ as the model bias and $\epivar(\rvgenstate, \rvgenact)$ as the epistemic variance. 
\end{definition}


%Introducing the notion of model error in \eqref{eq:error_proc} allows us to show that the uncertainty about $\ent (\rvmodnextstate | \rvgenstate = \genstate, \rvgenact = \genact) \geq \ent (\rvenvnextstate | \rvgenstate = \genstate, \rvgenact = \genact)$ with a derivation provided in Appendix \ref{app_ts_var}. This leads to the spread out data distribution in Figure \ref{fig:prob_statement_ts} which can result in the model hallucinating non-plausible transitions \cite{Jafferjee2020Jun}.



\subsection{Practical Mechanism}
\label{sec_ip_practice}
While the considerations above provide us with an information-theoretic perspective on error propagation, they leave us with the problem that neither $\rvenvnextstate$ nor $\Delta_t$ are known in practice. Thus, estimates of these quantities, based on the AES model's predictive distribution are required to make the theory above applicable to model-based rollouts.

We restrict model usage to a sufficiently accurate subset $\accsp \subseteq \statesp \times \actsp$, as proposed in \cite{Frauenknecht2024May}. Thus, we reformulate the notion of $\accsp$ to fit the Infoprop setting, i.e. $\accsp:= \left\{ (\genstate, \genact) \in \statesp \times \actsp \mid \ent(\rvpropnextstate) < \threshsingle, \modnextstate \sim \tskernel ( \cdot | \genstate, \genact ) \right\}$, with $\threshsingle$ the threshold of single-step information loss represented by $\ent(\rvpropnextstate)$. 
Within $\accsp$, we make the following assumptions:

\begin{assumption}
\label{assump:var_consistent}
The model's predictive variance $\modvar$ is a
    consistent estimator of $\envvar$ following the definition of \cite{Julier01}, i.e. \textcolor{red}{which follows from Definition \ref{def:error_process} i guess.}
    \begin{equation}
        \left( \modvar(\rvgenstate, \rvgenact) - \envvar(\rvgenstate, \rvgenact)\right) \succcurlyeq 0 
        \label{eq:consistent_var}
    \end{equation}
\end{assumption}

\begin{assumption}
\label{assump:unbiased}
    Within $\accsp$, the model bias $\modbias$ is negligible. Thus $\rvmodnextstate$ according to \eqref{eq:TS_prediction} is an unbiased estimator of $\rvenvnextstate$ according to \eqref{eq:env_prediction}, i.e.
    \begin{equation}
        \E \left[ \rvmodnextstate | \rvgenstate, \rvgenact \right] = \E \left[ \rvenvnextstate | \rvgenstate, \rvgenact \right]  \quad \text{if} \quad (\rvgenstate, \rvgenact) \in \accsp.
        \label{eq:no_bias}
    \end{equation}
\end{assumption}
Based on these assumptions, we consider individual samples from the parameter distribution $\rvparams \sim \distparams$ as noisy observations of the ground truth within $\accsp$. We construct our belief of the environment state from $E$ different realizations of the parameters $\rvparams = \params_t^1, \dots \params_t^E$ and combine the resulting predictive distributions in a manner akin to sensor fusion. As the different predictive distributions are assumed to be highly correlated, we use covariance intersection (CI) fusion \cite{Julier01} to estimate the environment's state
\begin{equation}
    \rvenvnextstate \approx \egtmean(\rvgenstate, \rvgenact) + \egtchol(\rvgenstate, \rvgenact)\rvenvale
    \label{env_state_estimate}
\end{equation}
with $\egtchol(\rvgenstate, \rvgenact)^\top \egtchol(\rvgenstate, \rvgenact) = \egtvar(\rvgenstate, \rvgenact)$, $\egtvar(\rvgenstate, \rvgenact) = \left( \frac{1}{E} \sum_{e=1}^{E} \modvarreal (\rvgenstate, \rvgenact)^{-1}\right)^{-1}$, and $\egtmean(\rvgenstate, \rvgenact) = \egtvar(\rvgenstate, \rvgenact)\left( \frac{1}{E} \sum_{e=1}^{E} \modvarreal (\rvgenstate, \rvgenact)^{-1} \modmeanreal (\rvgenstate, \rvgenact)\right)$. A visualization of the fusion step is provided in Figure \ref{fig:ci_fusion}.
\begin{figure}
     \centering
    \includegraphics[width=5cm]{figures/ci_fusion_v0.png}
    \caption{CI Fusion}
    \label{fig:ci_fusion}
 \end{figure}
 Further, an estimate of the model error distribution $\moderrordist$ is required. We consider $\modbias( \rvgenstate, \rvgenact) = 0$ based on Assumption \ref{assump:unbiased}. However, the epistemic variance
 \begin{equation}
     \epivar(\rvgenstate, \rvgenact) \approx \frac{1}{E} \sum_{e=1}^E \left( \modmeanreal(\rvgenstate, \rvgenact) - \egtmean (\rvgenstate, \rvgenact) \right) \left( \modmeanreal(\rvgenstate, \rvgenact) - \egtmean (\rvgenstate, \rvgenact) \right)^\top.
     \label{eq: epi_var_estimate}
 \end{equation}
 is approximated using the variance of predictive means concerning the fused mean.

 These approximations allow to use the framework introduced above in a practical rollout mechanism.
 %\end{comment}


==> sections/theory_backup.tex <==

\section{Infoprop Rollout Mechanism}

\subsection{General Setup}
\label{sec:ip_setup}
\begin{equation}
    \rvenvnextstate = \E_{\envkernel} \left[ \rvgennextstate | \rvgenstate=\genstate, \rvgenact=\genact, \rvenvale \right]
\end{equation}
\begin{equation}
    \rvmodnextstate = \E_{\tskernel} \left[ \rvgennextstate | \rvgenstate=\genstate, \rvgenact=\genact, \rvmodale \right]
\end{equation}
We introduce a dependence between environment transitions in \eqref{eq:env_prediction} and TS model predictions \eqref{eq:TS_prediction} by defining the following model error process.
\begin{definition}
    \label{def:error_process}
    We introduce a model error $\rvmoderror \sim \moderrordist$, such that $\rvmodnextstate = \rvenvnextstate + \Delta_t$. Thus, $\rvmoderror$ maps the uncertainty in the parameter space $\distparams$ to the output space of the model. In the following, we are solely concerned with the first two moments of $\moderrordist$, such that
    \begin{equation}
        \rvmodnextstate = \rvenvnextstate + \modbias(\rvgenstate, \rvgenact) + \epichol(\rvgenstate, \rvgenact) \rvmodepi
        \label{eq:error_proc}
    \end{equation}
    with $\epichol(\rvgenstate, \rvgenact)\epichol(\rvgenstate, \rvgenact)^\top = \epivar(\rvgenstate, \rvgenact)$ and $\rvmodepi \sim \gauss (0, I)$. We refer to $\modbias(\rvgenstate, \rvgenact)$ as the model bias and $\epivar(\rvgenstate, \rvgenact)$ as the epistemic variance.
\end{definition}

Further, We restrict model usage to a sufficiently accurate subset $\accsp \subseteq \statesp \times \actsp$, as proposed in \cite{Frauenknecht2024May}. We define $\accsp$ amenable to the Infoprop setting in Section \ref{sec:ip_stopping_roll} and make the following assumptions when operating in $\accsp$:

\begin{assumption}
\label{assump:var_consistent}
The model's predictive variance $\modvar$ is a
    consistent estimator of $\envvar$ following the definition of \cite{Julier01}, i.e. 
    $
        \left( \modvar(\rvgenstate, \rvgenact) - \envvar(\rvgenstate, \rvgenact)\right) \succcurlyeq 0 \quad \text{if} \quad (\rvgenstate, \rvgenact) \in \accsp.
    $
\end{assumption}

\begin{assumption}
\label{assump:unbiased}
    The model bias $\modbias$ is negligible. Thus $\rvmodnextstate$ according to \eqref{eq:TS_prediction} is an unbiased estimator of $\rvenvnextstate$ according to \eqref{eq:env_prediction}, i.e.
    $
        \E \left[ \rvmodnextstate | \rvgenstate, \rvgenact \right] = \E \left[ \rvenvnextstate | \rvgenstate, \rvgenact \right]  \quad \text{if} \quad (\rvgenstate, \rvgenact) \in \accsp.
    $
\end{assumption}

\subsection{Estimate Distributions}
\label{sec:ip_estimate_gt}
Assumptions \ref{assump:var_consistent} and \ref{assump:unbiased} allow us to interpret predictions under $\tskernel$ with different realizations of $\rvparams$ as noisy observations of the ground truth process under $\envkernel$. This insight allows us to address question \ref{item:ps_pred_dist} by providing a better estimate about $\rvenvnextstate$ when performing model-based rollouts.
 This perspective further allows to estimate $\moderrordist$ and make Definition \ref{def:error_process} applicable to a practical mechanism.

We construct our belief of the environment state from $E$ different realizations of the parameters $\rvparams = \params_t^1, \dots \params_t^E$ and combine the resulting predictive distributions in a manner akin to sensor fusion. As the correlation between different predictive distributions is unknown, we use covariance intersection (CI) fusion \cite{Julier01} with equal weighting to estimate the environment's state
\begin{equation}
    \rvenvnextstate \approx \rvegtnextstate = \egtmean(\rvgenstate, \rvgenact) + \egtchol(\rvgenstate, \rvgenact)\rvenvale
    \label{env_state_estimate}
\end{equation}
with $\egtchol(\rvgenstate, \rvgenact)^\top \egtchol(\rvgenstate, \rvgenact) = \egtvar(\rvgenstate, \rvgenact)$, $\egtvar(\rvgenstate, \rvgenact) = \left( \frac{1}{E} \sum_{e=1}^{E} \modvarreal (\rvgenstate, \rvgenact)^{-1}\right)^{-1}$, and $\egtmean(\rvgenstate, \rvgenact) = \egtvar(\rvgenstate, \rvgenact)\left( \frac{1}{E} \sum_{e=1}^{E} \modvarreal (\rvgenstate, \rvgenact)^{-1} \modmeanreal (\rvgenstate, \rvgenact)\right)$. A visualization of the fusion step is provided in Figure \ref{fig:ci_fusion}.
 
Next, we aim to estimate the model error distribution $\moderrordist$. We consider $\modbias( \rvgenstate, \rvgenact) = 0$ based on Assumption \ref{assump:unbiased}. The epistemic variance $\epivar(\rvgenstate, \rvgenact)$  is approximated using the variance of predictive means corresponding to different realizations of $\rvparams$ concerning the fused mean
 \begin{equation}
      \eepivar(\rvgenstate, \rvgenact) = \frac{1}{E} \sum_{e=1}^E \left( \modmeanreal(\rvgenstate, \rvgenact) - \egtmean (\rvgenstate, \rvgenact) \right) \left( \modmeanreal(\rvgenstate, \rvgenact) - \egtmean (\rvgenstate, \rvgenact) \right)^\top
     \label{eq: epi_var_estimate}
 \end{equation}
 as we interpret each realization $\modmeanreal$ a sample from the distribution $\moderrordist$.
 
\subsection{Quantify Corruption}
\label{sec:ip_uncertainty_acc}

Estimating $\rvegtnextstate$ and $\eepivar$ makes the error process \eqref{eq:error_proc} applicable to model-based rollouts.
This allows us to ask the question: \emph{How informative is a sample from the model about the corresponding realization of the environment state?} In information-theoretic notation this question yields the RV
\begin{equation}
    \rvpropnextstate := \E \left[ \rvegtnextstate | \rvgenstate=\genstate, \rvgenact = \genact, \rvmodnextstate=\modnextstate \right]
\end{equation}
which we refer to as the Infoprop (IP) state propagated by the IP kernel $\ipkernel(\cdot | \rvgenstate, \rvgenact, \rvmodnextstate) = \gauss\left(\propmean ( \rvgenstate, \rvgenact, \rvmodnextstate), \propvar( \rvgenstate, \rvgenact, \rvmodnextstate) \right)$. 
Following \eqref{eq:env_prediction} and \eqref{eq:error_proc}, an IP transition is described by
\begin{equation}
\begin{aligned}
    \rvpropnextstate =& \propmean ( \rvgenstate=\genstate, \rvgenact=\genact, \rvmodnextstate=\modnextstate) + \propchol ( \rvgenstate=\genstate, \rvgenact=\genact, \rvmodnextstate=\modnextstate) \rvcondun\\
    \text{with} \quad &\propmean(\genstate, \genact, \modnextstate) = \envmean(\genstate, \genact) + \kalgain(\genstate, \genact)\left( \envchol(\genstate, \genact) \envale + \epichol(\genstate, \genact) \modepi \right),\\
    &\propvar(\genstate, \genact, \modnextstate) = \left( I - \kalgain(\genstate, \genact) \right) \envvar(\genstate, \genact),\\
    &\kalgain(\genstate, \genact) = \envvar(\genstate, \genact) \left( \envvar(\genstate, \genact) + \epivar(\genstate, \genact)\right)^{-1},\\
\end{aligned}
    \label{eq:infoprop_state}
\end{equation}
$\propchol(\genstate, \genact) \propchol^\top (\genstate, \genact) = \propvar(\genstate, \genact)$, and $\rvcondun \sim \gauss (0, I)$.

Figure \ref{fig:ip_visualization} builds intuition for $\rvpropnextstate$.
We first consider the case where the model is perfect, i.e. $\Delta_t \sim \delta_0$, depicted in Figure \ref{fig:ip_perfect_model}. Here, a sample from the model $\modnextstate$ essentially gives the information about the realization of process noise $\envale$, as can be seen from the definition of $\propmean$ in \eqref{eq:infoprop_state}. Therefore, the realization of the environment state $\egtnextstate$ can be exactly identified, and the conditional entropy $\ent(\rvegtnextstate | \rvgenstate=\genstate, \rvgenact = \genact, \rvmodnextstate=\modnextstate) = \ent(\rvpropnextstate) = 0$ in the case of a perfect model.

In the general case of existent model error depicted in Figure \ref{fig:ip_noisy_model}, the sample from the model $\modnextstate$ leaves ambiguity about the distribution of $\rvegtnextstate$, as the model error corrupts the information. In this case $\ent(\rvegtnextstate | \rvgenstate=\genstate, \rvgenact = \genact, \rvmodnextstate=\modnextstate) = \ent(\rvpropnextstate)  > 0$
\footnote{\textcolor{red}{should be smth like $\log_2 (|\propvar|)$ or smth, right? we should maybe make this explicit. Probably not so easy due to the binning, but can we say it's proportional to something that depends on $\propvar$ and is greater than 0?}}
which corresponds to the information lost\footnote{In information-theoretic terms this rather corresponds to generated information but we believe this formulation is more intuitive from a MBRL practitioner's perspective.} due to using the faulty model for predicting the next state.
Thus, considering $\rvpropnextstate$ as a rollout variable allows us to trace back model error.

Most importantly, this effect extends to the multi-step prediction setting depicted in Figure \ref{fig:ip_multistep}. The information loss due to model error along a trajectory of length $T$
\begin{equation}
    \begin{aligned}
       & \ent \left( \bar{S}_1, \bar{S}_2, \dots \bar{S}_T | S_0 = s_0, A_0 = a_0, \hat{S}_1 = \hat{s}_1, \dots \hat{S}_T = \hat{s}_T \right)\\
       = & \sum_{t=0}^T \ent \left( \rvegtnextstate | \rvgenstate = \genstate, \rvgenact=\genact, \rvmodnextstate = \modnextstate \right) = \sum_{t=0}^T \ent \left( \rvpropnextstate \right)
    \end{aligned}
    \label{eq:gt_multistep_infoloss}
\end{equation}
is equivalent to the sum of entropies $\ent(\rvpropnextstate)$ along this path with a derivation in Appendix \ref{multistep_infoloss}.
\begin{figure}[tb]
     \centering
     \begin{subfigure}{0.22\textwidth} \includegraphics[width=\textwidth]{figures/ci_fusion_v0.png}
    \caption{CI Fusion}
    \label{fig:ci_fusion}
     \end{subfigure}
     \hfill
    \begin{subfigure}{0.22\textwidth} \includegraphics[width=\textwidth]{figures/infoprop_perfect_model_sketch_v0.png}
    \caption{Single step perfect model}
    \label{fig:ip_perfect_model}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.22\textwidth} \includegraphics[width=\textwidth]{figures/infoprop_noisy_model_sketch_v0.png}
    \caption{Single step noisy model}
    \label{fig:ip_noisy_model}
     \end{subfigure}
     \hfill
      \begin{subfigure}{0.22\textwidth} \includegraphics[width=\textwidth]{figures/infoprop_multistep_sketch_v0.png}
      \caption{Multistep}
      \label{fig:ip_multistep}
     \end{subfigure}
     \caption{Caption}
     \label{fig:ip_visualization}
 \end{figure}

 Consequently, propagating model-based rollouts with the IP kernel $\ipkernel$ instead of the TS kernel $\tskernel$ has two fundamental benefits. First, $\int_{\rvmodnextstate} \rvpropnextstate \, d\modnextstate\ \eqdist \rvegtnextstate $ by construction, i.e. IP rollouts follow the improved predictive distribution derived in Section \ref{sec:ip_estimate_gt} addressing question \ref{item:ps_pred_dist}. Second, the accumulated entropy of the IP state corresponds to data corruption due to model error which addresses question \ref{item:ps_data_corr}.

\subsection{Stopping Criteria}
\label{sec:ip_stopping_roll}
Having introduced how to propagate IP rollouts, the question remains when to terminate them. In the following, we propose two termination criteria.

First, IP rollouts build on the assumption that model-based rollouts are performed in a sufficiently accurate subset $\accsp \subseteq \statesp \times \actsp$. Following the ideas of \cite{Frauenknecht2024May}, we construct $\accsp$ on the notion of single-step predictive uncertainty.
Thus, we define $\accsp:= \left\{ (\genstate, \genact) \in \statesp \times \actsp \mid \ent(\rvpropnextstate) \leq \threshsingle, \modnextstate \sim \tskernel ( \cdot | \genstate, \genact ) \right\}$ amenable to the Infoprop setting, with $\threshsingle$ the threshold of single-step information loss represented by $\ent(\rvpropnextstate)$. Consequently, IP rollouts are terminated, whenever $\ent(\rvpropnextstate) > \threshsingle$ to enforce operation in $\accsp$.

Second, accumulating smaller errors can corrupt the data distribution of long model rollouts. Thus, we define an upper bound on cumulative information loss $\sum \ent(\rvpropnextstate) \leq \threshmulti$ to avoid data corruption.

Heuristics for determining values of $\threshsingle$ and $\threshmulti$ depend on the class of AES model and MBRL algorithm at hand. An example is provided in Section \ref{sec:ip_dyna_alg}. Combining the steps above yields the Infoprop rollout mechanism illustrated in Algorithm \ref{alg:infoprop_rollout}.

 \begin{algorithm}
\caption{Infoprop (needs to be done)}
\begin{algorithmic}
    \Require Policy $\pi (\cdot | \rvgenstate)$, ASM model $f(\rvparams, \rvgenstate, \rvgenact, \rvmodale)$, start state $s_0$, thresholds $\threshsingle, \threshmulti$, max length $T$
    \State 
    \While{$t<T+1$}
    \State $\genact \sim \pi(\cdot | \genstate)$
    \State $\modale\sim \gauss(0, I)$
    \For{$e=1, E$}
    \State $\theta_e \sim \distparams$
    \EndFor
    \EndWhile
    \State todo
\end{algorithmic}
\label{alg:infoprop_rollout}
\end{algorithm}




 
